Performance Bounds of Model Predictive Control for Unconstrained and Constrained Linear Quadratic Problems and Beyond

We study unconstrained and constrained linear quadratic problems and investigate the suboptimality of the model predictive control (MPC) method applied to such problems. Considering MPC as an approximate scheme for solving the related fixed point equations, we derive performance bounds for the closed-loop system under MPC. Our analysis, as well as numerical examples, suggests new ways of choosing the terminal cost and terminal constraints, which are \emph{not} related to the solution of the Riccati equation of the original problem. The resulting method can have a larger feasible region, and cause hardly any loss of performance in terms of the closed-loop cost over an infinite horizon.

==> recycle.tex <==

In the context of MPC, an optimization problem is solved at each stage to make the control selection. Therefore, the term \emph{optimality} may refer to the solutions obtained in each stage with respect to the optimization problem \cite{scokaert1999suboptimal}. In our discussion, however, we assume the optimization problem associated with MPC is solved exactly at each time. Instead, we are interested in the performance of MPC compared with the optimal control to the original optimal control problem. For an LQR problem, the optimal control is well-known, and we use it as a test-bed to evaluate the suboptimality of the control law produced by MPC measured by the accumulated cost of the closed-loop system over infinite stages. The magnitude of the suboptimality is bounded by what we referred to as the \emph{performance bounds}. The intuition obtained for LQR will be carried further to constrained LQR as well as nonlinear systems, where the optimal control cannot be obtained analytically.



We provide two examples. In the first scalar example, we show the bound \eqref{eq:lqr_b_monotone} and the Newton step interpretation by plotting the Bellman curve of LQR and demarcate the values of $K^*$, $K_{\Tilde{L}}$, $F(\overline{K})$, as well as $F_{L^*}(\overline{K})$. In the second example, we consider two dimensional and four dimensional LQR problems and list the performance bounds as well as the actual performance.




